On Quantum Natural Policy Gradients

This research delves into the role of the quantum Fisher Information Matrix (FIM) in enhancing the performance of Parameterized Quantum Circuit (PQC)-based reinforcement learning agents. While previous studies have highlighted the effectiveness of PQC-based policies preconditioned with the quantum FIM in contextual bandits, its impact in broader reinforcement learning contexts, such as Markov Decision Processes, is less clear. Through a detailed analysis of L\"owner inequalities between quantum and classical FIMs, this study uncovers the nuanced distinctions and implications of using each type of FIM. Our results indicate that a PQC-based agent using the quantum FIM without additional insights typically incurs a larger approximation error and does not guarantee improved performance compared to the classical FIM. Empirical evaluations in classic control benchmarks suggest even though quantum FIM preconditioning outperforms standard gradient ascent, in general it is not superior to classical FIM preconditioning.

==> tex_files/npg_pqc.tex <==
\section{Smoothness of PQC-based policies}\label{sec: NPG-PQC}

  The regret lemma presented in this section follows essentially the regret lemma proposed in \cite{agarwal_theory_2021}, restated here for completeness. The NPG-PQC regret lemma \ref{lemma: NPG-PQC regret lemma} follow from the smoothness of the PQC-generated policies. 
  
  \begin{lemma}{NPG Regret Lemma \cite{agarwal_theory_2021}}{l}
    \label{lemma: NPG regret lemma}
    Fix a comparison policy $\tilde{\pi}$ and a state distribution $\rho$. Assume for all $s \in \mathcal{S}$ and $a \in \mathcal{A}$ that $\log \pi(a \mid s,\theta)$ is a $\beta$-smooth function of $\theta$. consider $\pi^{(0)}$ the uniform distribution for every state and the sequence of weights $w^{(0)}, \ldots, w^{(T)}$ satisfying $\left\|w^{(t)}\right\|_2 \leq W$. Let $\epsilon_t$ be the approximation error at time $t$:

    \begin{equation}
      \epsilon_t=\mathbb{E}_{s \sim \tilde{d}} \mathbb{E}_{a \sim \widetilde{\pi}(\cdot \mid s)}\left[A^{(t)}(s, a)-w^{(t)} \cdot \nabla_\theta \log \pi^{(t)}(a \mid s)\right]
    \end{equation}
    Then the regret is upper bounded by:
    \begin{equation}
        \min _{t<T}\left\{V^{\tilde{\pi}}(\rho)-V^{(t)}(\rho)\right\} \leq \frac{1}{1-\gamma}\left(\frac{\log |\mathcal{A}|}{\eta T}+\frac{\eta \beta W^2}{2}+\frac{1}{T} \sum_{t=0}^{T-1} \epsilon_t\right)
    \end{equation}
\end{lemma}
  
  Recall that a function $f$ is called $\beta$-smooth if $\forall x,x' \in \mathbb{R}^d$:
  \begin{equation}
    \lVert \nabla f(x) -  \nabla f(x') \rVert_2 \leq \beta \lVert x' - x \rVert_2^2
    \label{eq: smoothness}
  \end{equation}
  which, via Taylor's theorem implies:

  \begin{equation}
    \lvert f(x') - f(x) - \nabla f(x) (x' - x) \rvert \leq \frac{\beta}{2} \lVert x' - x \rVert_2^2
  \end{equation}

  Lemma \ref{lemma: softmax smoothness} states the smoothness of the softmax policy.

  \begin{lemma}
    \label{lemma: softmax smoothness}
    Let $\pi(a|s,\theta)$ be an \textit{arbitrary} $n$-qubit parameterized softmax policy (Definition \ref{def: softmax policy}). Let $|A|$ be the total number of actions of a given environment and $M$ the upper bound on the expectation value of a given observable $O_a$ representing the numerical preference of action $a$. Then, the log policy is $|A|M^2$-smooth. 
 \end{lemma}

 \begin{proof}
  For simplicity, the policy is represented as $\pi_{\theta}$.
  \begin{align}
  \lVert &\nabla \log \pi_{\theta} -  \nabla \log \pi_{\theta'} \rVert_2 \nonumber \\
  &\leq \lvert \nabla_{\theta} \langle O_a \rangle_{\theta} - \nabla_{\theta} \langle O_a \rangle_{\theta'} \rvert + \lvert\sum_{a'} \nabla_{\theta} \langle O_a \rangle_{\theta} - \sum_{a'} \nabla_{\theta} \langle O_a \rangle_{\theta'}\rvert \nonumber\\
  &\leq \lvert \nabla_{\theta} \langle O_a \rangle_{\theta} - \nabla_{\theta} \langle O_a \rangle_{\theta'} \rvert + \sum_{a'} \lvert \nabla_{\theta} \langle O_a \rangle_{\theta} - \nabla_{\theta} \langle O_a \rangle_{\theta'}\rvert \nonumber\\
  \label{eq: smoothness log softmax}
  \end{align}

  Recall that the expectation value of a given observable $\langle O_a \rangle_{\theta}$ can be written as a sine function of a single trainable parameter $\theta$ as in Lemma \ref{lemma: softmax log policy gradient}. Thus, the derivative of the expectation value is given by $\partial_{\theta} \langle O_a \rangle_{\theta} = A \cos (\theta + B)$ and,

  \begin{align}
    \lvert \nabla_{\theta} \langle O_a \rangle_{\theta} - \nabla_{\theta} \langle O_a \rangle_{\theta'} \rvert &= \lvert A \bigl( \cos(\theta + B) - \cos(\theta' + B) \bigr) \rvert \nonumber \\
    &= A^2 \lvert \bigl( \cos(\theta + B) - \cos(\theta' + B) \bigr) \rvert
  \end{align}
  Thus, from mean value theorem, $\exists c \in (\theta + B , \theta' + B)$ s.t
  \begin{align}
    A^2 \lvert \bigl( &\cos(\theta + B) - \cos(\theta' + B) \bigr) \rvert = \nonumber\\
    &=A^2 \lvert \bigl( -\sin(c) (\theta + B - \theta' - B ) \bigr) \rvert \leq A^2|\theta - \theta'|
  \end{align}
  Substituting this in Equation \ref{eq: smoothness log softmax},

  \begin{equation}
    \lVert \nabla \log \pi_{\theta} -  \nabla \log \pi_{\theta'} \rVert_2 \leq A_a^2|\theta - \theta'| + \sum_{a'} A_{a'}^2|\theta - \theta'|
  \end{equation}
  where $A_a$ is the amplitude associated to the sine function after decomposition of the expectation value of the observable associated to action $a$. Since it is considered that $O_a \neq O_a'$ then $A_a \neq A_a'$.\\
  Let every observable be composed of $M$ terms and $A_a$ follow Equation \ref{eq: ABC expval decomposition}. Then,
  \begin{equation}
    \langle O_a \rangle_{\theta} = \sum_{m=0}^{M-1} \langle O_a^m \rangle_{\theta} \in [-m, m] \quad \rightarrow \quad A_a \leq \frac{M}{2}\sqrt{2}
  \end{equation}
  Thus, 
  \begin{equation}
    \lVert \nabla \log \pi_{\theta} -  \nabla \log \pi_{\theta'} \rVert_2 \leq |A|M^2 |\theta - \theta'| 
  \end{equation}
  completing the proof.
 \end{proof}

 Lemma \ref{lemma: Born smoothness} states the smoothness of the generalized Born policy.

 \begin{lemma}{Smoothness of the generalized Born policy}{l}
  \label{lemma: Born smoothness}
  Let $\pi(a|s,\theta)$ be an \textit{arbitrary} $n$-qubit parameterized Born policy (Definition \ref{def: born policy}). Let $|A|$ be the total number of actions of a given environment and $V_a$ be the partition associated to action $a$. Then, the log policy is $\frac{|V_a|}{4}$-smooth. 
\end{lemma}

\begin{proof}
  For simplicity consider the policy represented as $\pi_{\theta} = \langle P_a \rangle_{\theta}$.
  
  \begin{equation}
    P_a = \sum_{v \in V_a} |v\rangle \langle v| \ \rightarrow \ \langle P_a \rangle_{\theta} = \langle \psi(s,\theta) | \sum_{v \in V_a} |v\rangle \langle v| \psi(s,\theta) \rangle = \sum_{v \in V_a} \langle P_v \rangle_{\theta}
  \end{equation}
  where $\langle P_v \rangle_{\theta}$ ca be written as a sine function (Equation \ref{eq: ABC expval decomposition}). 
  \begin{equation}
    \langle P_a \rangle_{\theta} = \sum_{v \in V_a} A_v \sin(\theta + B_v) + C_v \quad \rightarrow \quad \nabla_{\theta} \langle P_a \rangle_{\theta} = \sum_{v \in V_a} A_v \cos(\theta + B_v)
  \end{equation}
  Thus, the log policy gradient becomes unbounded as:
  \begin{equation}
    \nabla_{\theta} \log \langle P_a \rangle_{\theta} = \frac{\nabla_{\theta} \langle P_a \rangle_{\theta}}{\langle P_a \rangle_{\theta}} = \frac{\sum_{v \in V_a} A_v \cos(\theta + B_v)}{\sum_{v \in V_a} A_v \sin(\theta + B_v) + C_v}
  \end{equation}
  For that reason, let us consider a clipped version of the log policy gradient: 
  \begin{equation}
    \tilde{\nabla}_{\theta} \log \langle P_a \rangle_{\theta} = \nabla_{\theta} \log \langle P_a \rangle_{\theta} \sum_{v \in V_a} A_v \sin(\theta + B_v) + C_v = \sum_{v \in V_a} A_v \cos(\theta + B_v)
  \end{equation}
  Using the clipped log policy gradient,
  \begin{align}
    \lVert \tilde{\nabla}_{\theta} \log \langle P_a \rangle_{\theta} - \tilde{\nabla}_{\theta} \log \langle P_a \rangle_{\theta'} \rVert_2 &\leq | \sum_{v \in V_a} A_v \cos(\theta + B_v) - \sum_{v \in V_a} A_v \cos(\theta' + B_v)| \nonumber \\
    &\leq \sum_{v \in V_a}|A_v\cos(\theta + B_v) - A_v\cos(\theta' + B_v)| \nonumber \\
    &\leq \sum_{v \in V_a} A_v^2 |\theta - \theta'| \nonumber \\
    &\stackrel{(a)}{\leq} \frac{|V_a|}{4}|\theta - \theta'|
  \end{align}
  where:
  (a) follows from the upper bound taking the definition of $A_v$ as in Equation \ref{eq: ABC expval decomposition}.
\end{proof}

Therefore, the NPG-PQC Regret Lemma can be stated using the smoothness properties of the Softmax and generalized Born policies.

\begin{lemma}{NPG-PQC Regret Lemma}{l}
  \label{lemma: NPG-PQC regret lemma}
  Fix a comparison policy $\tilde{\pi}$ and a state distribution $\rho$. Consider $\pi^{(0)}$ the uniform distribution for every state and the sequence of weights $w^{(0)}, \ldots, w^{(T)}$ satisfying $\left\|w^{(t)}\right\|_2 \leq W$. Let $\epsilon_t$ be the approximation error at time $t$:

  \begin{equation}
    \epsilon_t=\mathbb{E}_{s \sim \tilde{d}} \mathbb{E}_{a \sim \widetilde{\pi}(\cdot \mid s)}\left[A^{(t)}(s, a)-w^{(t)} \cdot \nabla_\theta \log \pi^{(t)}(a \mid s)\right]
  \end{equation}
  Let $\log \pi(a \mid s,\theta)$ be the Softmax policy (Definition \ref{def: softmax policy}). From Lemma \ref{lemma: softmax smoothness},the log policy is a $|A|M^2$-smooth function of $\theta$, then the regret is upper bounded by:
  \begin{equation}
      \min _{t<T}\left\{V^{\tilde{\pi}}(\rho)-V^{(t)}(\rho)\right\} \leq \frac{1}{1-\gamma}\left(\frac{\log |\mathcal{A}|}{\eta T}+\frac{\eta |A|M^2 W^2}{2}+\frac{1}{T} \sum_{t=0}^{T-1} \epsilon_t\right)
  \end{equation}
  Moreover, let $\log \pi(a \mid s,\theta)$ be the generalized Born policy (Definition \ref{def: born policy}). From Lemma \ref{lemma: Born smoothness},the log policy is a $\frac{|V_a|}{4}$-smooth function of $\theta$, then the regret is upper bounded by:
  \begin{equation}
      \min _{t<T}\left\{V^{\tilde{\pi}}(\rho)-V^{(t)}(\rho)\right\} \leq \frac{1}{1-\gamma}\left(\frac{\log |\mathcal{A}|}{\eta T}+\frac{\eta |V_a| W^2}{4}+\frac{1}{T} \sum_{t=0}^{T-1} \epsilon_t\right)
  \end{equation}
\end{lemma}

==> tex_files/related_work.tex <==
\section{Related Work}\label{sec: related work}
